Predicting and Explaining Human Semantic Search in a Cognitive Model

Recent work has attempted to characterize the structure of semantic memory and the search algorithms which, together, best approximate human patterns of search revealed in a semantic fluency task. There are a number of models that seek to capture semantic search processes over networks, but they vary in the cognitive plausibility of their implementation. Existing work has also neglected to consider the constraints that the incremental process of language acquisition must place on the structure of semantic memory. Here we present a model that incrementally updates a semantic network, with limited computational steps, and replicates many patterns found in human semantic fluency using a simple random walk. We also perform thorough analyses showing that a combination of both structural and semantic features are correlated with human performance patterns.

==> 06-ignore_text.tex <==
%%00

\ignore{\author{
{\large \bf Filip Miscevic \\Cognitive Science Program\\Indiana University Bloomington\\fmiscevi@umail.iu.edu}
\And {\large \bf Aida Nematzadeh\\Department of Psychology\\University of California, Berkeley 
\\nematzadeh@berkeley.edu}
\And {\large \bf Suzanne Stevenson\\Department of Computer Science\\University of  Toronto\\suzanne@cs.toronto.edu}
}
}

\ignore{
We need to understand the properties of an incrementally-developed semantic memory organization, and whether it is sufficiently robust to support a very simple search process, or if a more complex algorithm is required to achieve observed human performance.

%
We show that a semantic structure created incrementally within an online word learning model can yield human performance in semantic search using a simple random walk.
}
%
%
While the requirements of human semantic search presumably influence how semantic memory is organized, the structure of semantic memory also must be shaped by the incremental processes of language acquisition. 

\ignore{One reviewer suggested that we indicate here what the features were.}
\ignore{
Free recall in semantic memory has been likened to that of foraging through patches in semantically related words,

Recent experiments on free recall in semantic memory have led to the hypothesis that people forage through semantically related patches of words, in much the same way as an animal might forage in its habitat for resource-rich patches. \citeA{hills.etal.2015} suggest that such a patch in semantic memory is best described as , strict category boundaries.

Building on previous work, we show that  from naturalistic language use online (i.e. during the process of learning). Furthermore, 
}

%%01
\ignore{
\begin{verbatim}
DONE 1.	Semantic memory – representation and processing – is an important area of study. Ties in to mental lexicon, conceptual representations. [Prior to current first paragraph – why do we care about this area of study?] – look at ignore text

DONE 2.	The semantic fluency task gives psychologists a way to reveal aspects of semantic representation and the processing algorithms that access it. See an exploit/explore pattern of enumerating subcategories.

DONE 3.	Recent work has explored the interdependence and trade-offs between types of semantic representation and processing – accounting for human behavior in a semantic fluency task can be achieved through:

 a.	Either a simple representation [vector-based] and an informed algorithm [2-stage]. (Hills et al.)

 b.	Or a richer representation [semantic network] and a simple algorithm [random walk]. (Abbott et al., Nematzadeh et al.)

DONE 4.	How do we choose between(3a) and (3b) if the components are interdependent and both combinations account for the data?

 a.	A priori, would prefer a solution in which a simple algorithm operates over a structured representation: Having a simple process is beneficial for efficient access. (The reasoning here is that the cost of structuring representation happens when words are learned, rather than having a less efficient algorithm where the cost is incurred on every access. But note that in our word learner, “learning” happens every time you encounter a word. So, this might not be the obvious trade-off you think.)
 i.	Other evidence that semantic memory is structured: MillerFellbaum91

 b.	Data driven: Both (3a) and (3b) have been shown to account for IRT patterns; data thus far doesn’t distinguish.
 i.	But could look at other aspects of the human data to see if the (3b) approach can account for other things beyond IRT, to give more support.

DONE 5.	Given (3b), how do we choose among the possible representations? – Learnability.
 a.	Norms – not clear.
 b.	BEAGLE – learnable but not incrementally from reasonable data.
 c.	Word Learner – learns from reasonable data, but not yet shown that an incrementally-created sem net would have right properties.

DONE 6.	This paper:
 a.	Show a sem net created incrementally within a word learner can show IRT pattern.
 b.	Show it can account for additional human data.
 c.	Further analyze the properties of the representations that enable the IRT pattern.

\end{verbatim}
\todo{Use the term `semantic fluency' throughout the paper: not free recall. Check it doesn't say `free recall' anywhere.} \fm{I fixed this.} }% end ignore verbatim text

\sxs{I noticed you took out the spaces between long dashes and the words next to them -- eg, just below you replaced `memory -- word... storage -- is' with `memory--word... storage--is'.  This isn't correct Latex:  You need to have three `-'s in a row if you want to do this.  The way it is now, `memory--word' is the syntax used for a two-word phrase, like `word---meaning associations', so these are very difficult to read now (actually, they simply read incorrectly).  You either need to put the spaces back, or change these to `---' (without changing any word--word pairs that are supposed to be that way) -- i.e., you can't just do a global search and replace all, you have to check them.}\fm{I fixed this, a single-dash (-) is fine for word-word pairs, isn't it? That's how word-word pairs were written, anyways}

\ignore{ \sxs{What did Abbott et al. say to this issue?} \fm{They said that experiments need to be designed to specifically tease out the differences.} } 

\ignore{
At this stage, it is important to seek additional evidence of such an approach---i.e., a simple random walk over a structured semantic network---by seeing if it can account for further aspects of the empirical data available on semantic fluency.
%
This is one of the goals of the current paper.
}

\ignore{
\fm{I don't think we need this next paragraph since we clearly state what we are asking and testing in the pragraph that comes after. Also, we've already mentioned that the simple approach works - the wording here is what confused some reviewers last time.}
To fully understand the interaction of semantic representation and search, we need to study the properties of an incrementally-developed semantic memory organization, and whether it is sufficiently robust to support a very simple search process, or if a more complex algorithm is required to achieve observed human performance.
%
Moreover, while the requirements of human semantic search presumably influence how semantic memory is organized,
the structure of semantic memory must also be shaped by the incremental processes of language acquisition.
}

%
\ignore{
This is different from \citeA{nematzadeh.etal.2016} in that here the network is created while the word representations are being learned, not afterward. \sxs{Do we still need the last sentence?}\fm{I agree, we specifically indicate this is a departure from previous work above.}
}

\ignore{ % begin ignore old text from Aida.

\citeauthor{hills.etal.2012} suggest that accounting for this data requires an informed search process that decides when to continue searching (exploiting) within a subcategory, and when to switch to a new one (exploring). 
%
Specifically, they model the observed human behavior by applying this search algorithm on simple \sxs{It's not clear to me that we need the following detail of their algorithm in the intro.}
local cues, such as word similarity, guide searching within subcategories, and global cues, such as word frequency, determine a switch into new subcategories.
To test their hypothesis, \citeauthor{hills.etal.2012} use a simple vector-space model based on word co-occurrence frequency.

By contrast, \citeA{abbott.etal.2015} construct a richer semantic representation---a semantic network based on human association norms \cite{nelson.etal.1998}---in which words are represented as nodes and the similarities between them are represented with weighted edges. They show that a simple search algorithm over the network, a random walk, can also produce the observed human pattern.
%
\citeA{nematzadeh.etal.2016} further show that a simple random walk over the simple vector-based representations used by \citeauthor{hills.etal.2012} can mimic the human search pattern, as long as those representations are structured into a semantic network.
%

Given the dependence between the choice of representation and type of search, two important questions remain unexplored: which representation best approximates human knowledge, and how these representations are learned. \citeA{hills.etal.2012} assume that vector-space representations based on co-occurrence frequencies capture how people process \sxs{``encode''?} similarly judgments, but this assumption has been criticized \sxs{``challenged''?} \cite{griffiths.etal.2007}. \sxs{Criticized why?} Also, the vector-space model is trained on Wikipedia data, which is arguably not a good proxy for the linguistic input that people are exposed to in learning their semantic lexicon. By contrast, \citeA{abbott.etal.2015} directly use human associations norms as the basis for their representation, so that their semantic network does accurately reflect human judgments of word relatedness. However, it is not clear how the similarity assessments captured in such norms are learned through exposure to language.
%
\citeA{nematzadeh.etal.2016} aim to address some of these limitations by using word representations learned by a cognitive model from a corpus of naturalistic language use.
%They create a semantic network by comparing all word pairs and connecting the ones whose similarity exceeds a threshold. 
They demonstrate that a simple random walk over a semantic network formed from these learned representations can predict the semantic fluency data as in \citeA{hills.etal.2012} and \citeA{abbott.etal.2015}.

****************************
\sxs{I'm here in working on the intro. Stopping for tonight. 10:08pm, Sept 6.}

However,
%

The combination of a structured representation and simple search is favorable (compared to a simple representation and a complex search); because it can decrease the cognitive load associated with the retrieval of information (\todo{cite? can justify?}).
%
While the requirements of human semantic search presumably influence how semantic memory is organized,
the structure of semantic memory must also be shaped by the incremental processes of language acquisition. 
%
In particular, children simultaneously learn word meanings as well as the relations between them \cite{jones.etal.1991}. 
%
This has been ignored by all the previous work discussed so far; when they learn the semantic representation it only includes word representations and not their relations. The semantic network is created by simply comparing the word representations after training and not through the process of learning representations.
%
To fully understand the interaction of semantic representation and search, we need to study the properties of an incrementally-developed semantic memory organization, and whether it is sufficiently robust to support a very simple search process, or if a more complex algorithm is required to achieve observed human performance.



Our contributions are threefold:
%
First, we show that a semantic network created incrementally within an online word learning model---from naturalistic child language acquisition data---can yield human performance in semantic search using a simple random walk. This is different form \citeA{nematzadeh.etal.2016} in that we do not assume that the network is created after but at as the word representations are learned.
%
This confirms that a semantic network created and updated incrementally--- while the model is learning---has the appropriate structure to yield patterns observed in semantic fluency task, despite having noisy and incomplete connections as a result of being generated from partial knowledge acquired at each time step. 
%
Second, new data
\todo{Finish}
%
Third, we go beyond previous analyses of semantic organization to determine more precisely the network properties that are correlated with human performance patterns.
We find that the \textit{both} structural and semantic properties are necessary to generate patterns observed in human semantic fluency data.


} % end ignore old text from Aida.

%%02
%
%\ignore{
%\an{use semantic features instead of WordNet hypernyms and add a footnote to cite where the features are taken.
%There are more resources than WordNet.}
%}
%


\ignore{
\SXS{I tried to clean up the text in the next paragraph, but it's not clear to me why we're spending time talking about the representation of contextual features in the meaning probabilities.  We don't mention the impact of that on our semantic networks, do we?  Anyway, it's fine to leave it here, but if we ended up needing space, could cut the part on contextual features and just leave the conceptual hierarchy part.} \fm{You're right, the main reason I included it is to show that the model is doing more than just acquiring the gold meanings, and its ability to include information about context adds to its plausbility as as cognitive model.}
}

 \ignore{through shared features across words. The learned meaning probabilities reflect such semantic similarities across related words. \fm{Personally I am not sure what this means.} 
Moreover, as a consequence of capturing statistically co-occurring features for a given word, the model also learns associations of contextual features with a word.
%learns not only the features associated with that particular word, but features that often occur in the same context as the word. 
For example, in the above utterance-scene pair, the model may come to associate a non-zero probability to the feature \textsc{body-of-water}, as the context in which the word crocodile is spoken may also contain referents to its surroundings, \eg rivers. Hence, the learned meanings of words capture not only a conceptual hierarchy for that word but also information about the context of their usage.
}

\ignore{\sxs{This next sentence doesn't make sense here: it's not clear what processes it's talking about.  Doesn't capture the line of reasoning in the notes in the Latex file.  Either remove the sentence or spell it out better.} Therefore, it is not a realistic cognitive assumption for these processes to occur independently of each other.} 

\ignore{is possible to compute the similarity of two learned word vectors $\mathbf{x}$ and $\mathbf{y}$ by calculating their cosine distance:
\begin{align*}
    similarity &= \frac{\mathbf{x}\cdot \mathbf{y}}{\lVert \mathbf{x} \rVert \lVert \mathbf{y} \rVert}
\end{align*}
\noindent
}

\ignore{
Following \citeA{anderson.matessa.1992}, we use a Bayesian framework to calculate the probability that word $w$ belongs to cluster $k$. Recall that the meaning of a word is represented $P(\cdot | w)$ which is stored in a vector, $F$. Then, by Bayes' rule,
%
\begin{align*}
    P(k|F) &= \frac{P(F|k)P(k)}{\sum_{k'}P(F|k')P(k') }
\end{align*}
%
\textbf{Prior.} The probability of a word $n+1$ being assigned to cluster $k$ is expressed by the prior
\begin{align*}
    P(k) &=  \begin{cases} 
      \frac{n_k}{n+\alpha} & n_k>0 \\
      \frac{\alpha}{n+\alpha} & n_k=0 \text{ (new cluster)} 
   \end{cases}
\end{align*}
%
Here, $n_k$ is the cardinality of cluster $k$, $n$ is the number of words observed so far, and the parameter $\alpha$ determines the likelihood of creating a new cluster. When $n_k>\alpha$, the formation of new clusters becomes unlikely and the formation of larger clusters is favored. This ensures that there must be fewer categories than there are words, a basic feature of categorization.\\
%
\textbf{Likelihood.} \fm{How much detail is needed here? There's a fairly lengthy derivation here in the EMNLP paper..}
}

\sxs{Given that we talk about semantic similarity in the intro as important to semantic networks, it's important to add (back) something here about how the representation captures semantic similarity among words.} \fm{How about this:} 

%%031
%----- ignored text
\ignore{
Under this assumption, efficient free recall depends on an optimal policy for when to continue searching (exploiting) within a patch, and when to switch to a new one (exploring).
In modelling this behavior, Hills et al.\ use a simple vector-based semantic representation, BEAGLE \cite{jones.etal.2007}, a spatial vector model trained on the Wikipedia corpus. Simulation of semantic fluency then proceeds using a two-stage search algorithm on the learned vectors: local cues, such as similarity, are used to search within clusters, and global cues, such as the frequency with which a word appears, are used to switch into new patches \cite{hills.etal.2012}.
}%----- ignored text




\ignore{
%\SXS{The differences don't look that different between learner and BEAGLE.  What seems different in the learner is that the cosine continues to increase \textbf{after} a patch switch--that seems odd to me.  I don't understand how that can happen.} \fm{I think I figured it out! After wracking my brain and painstakingly verifying there were no code bugs (which there weren't!) I realized my intuition that `animal' being compared with another word would bring down the average cosine similarity on the second patch entry position was correct! What I failed to consider is that this will happen at the beginning of EVERY walk in the trial. When I exclude the first cluster retrieved in continuity with `animal', the discrepancy is lessened.} 
%
Note, as mentioned before, that the `human' data in \Figure{fig:hillscos} is calculating cosine similarities over the BEAGLE representations of the words generated by participants in the free recall task; thus the patterns observed in Figures \ref{fig:hillscos} and \ref{fig:beaglecos} may have a strong resemblance since they are using the same vector space.
\SXS{I'm not really sure where this last sentence fits in, or even if it does--depends on what you say about the match of our models to the human data.}
}

\ignore{
We note that although \citeA{hills.etal.2012} found that randomly sampling words without replacement in BEAGLE did not fit the human data, we show  that when the representation is structured into a semantic network and the appropriate threshold for cosine similarity is chosen, it fits the data on all of the measures we investigated as well as our models do.





\begin{enumerate}
    \item Performance of incremental networks (figure 1)
    \begin{itemize}
        \item rather than generating the semantic networks on the final learned word vectors, we can update the semantic network online as the model learns
        \item trained on 78k utterances from the training scene/utterance pairs derived from CHILDES
        \item IRT pattern is reproduced
    \end{itemize}
    \item Logistic regression on features
    \begin{itemize}
        \item sample equally from the parameter spaces in which IRT patterns occur and do not occur (so null model classification rate would be $50\%$)
        \item for each of the different models (gold, learner, beagle),  perform logistic regression on all possible combinations of the following features: number of vertices (V), number of edges (E), characteristic path length (L), L normalized to an equivalent Erdos-Renyi graph (lambda), clustering coefficient (CC), CC normalized to an equivalent Erdos-Renyi graph (gamma), sparsity, small-worldness (sigma), adjusted rand index, F-score weighted by cluster sizes, unweighted F-score, number of clusters determined by HDBSCAN, number of clusters determined by the naive clustering algorithm (i.e., deleting the word 'animal' and examining the disconnected components), number of singletons (i.e., number of words that are only connected to 'animal')
        \item examine simplest models that achieve the highest
        \begin{enumerate}
            \item overall classification score - percent of all graphs trained on that are correctly classified as having the IRT pattern or not
            \item true positives score - percent of IRT-producing graphs that are correctly classified (I looked at this separately because initially there were more non-IRT graphs than IRT graphs when the parameter space is unformly sampled)
            \item leave-one-out (LOO) cross-validation score (CV) - make n partitions on the data that leave one graph out, and take the average score of whether that graph is classified correctly or not
            \item stratified k-fold (SKF) cross-validation score - split training data into k equally sized partitions that also capture relative frequencies of each category. Used $k=3$
        \end{enumerate}
        \item Logistic regression results:
        \begin{enumerate}
            \item Gold
            \begin{itemize}
                \item trained on 38 each of IRT and non-IRT graphs
                \item best model: $|E|$, L, $\gamma$, $\sigma$, \# of singletons, precision and F-score (on the naive clustering algorithm)
                \item classification accuracy: 0.96
                \item LOO CV: 0.91
                \item SKF CV: 0.84
                
                \item second best model: $|E|$, L, CC, $\gamma$, $\sigma$, \# of singletons, precision (on the naive clustering algorithm)
                \item classification accuracy: 0.96
                \item LOO CV: 0.91
                \item SKF CV: 0.84
            \end{itemize}
            \item BEAGLE
            \begin{itemize}
                \item trained on 33 each of IRT and non-IRT graphs
                \item best model: $|E|$, weighted F-score (HDBSCAN)
                \item classification accuracy: 0.86
                \item LOO CV: 0.81
                \item SKF CV: 0.69
                \item model with just edges (or edges and sparsity) achieves LOO CV of 0.80, but same classification and SKF score
            \end{itemize}
            \item Learner
            \begin{itemize}
                \item trained on 21 IRT-producing graphs, 21 non-IRT graphs
                \item best model: $|E|$, \# clusters determined by HBDSCAN, \# singletons
                \item classification accuracy: 0.95
                \item LOO CV: 0.95
                \item SKF CV: 0.86
                \item second best model: $|V|$, $|E|$, \# singletons
                \item classification accuracy: 0.95
                \item LOO CV: 0.95
                \item SKF CV: 0.79
            \end{itemize}
              \an{I wonder why the number of edges is enough in predicting the IRT data. I expected CC would be important. Are not we overfitting the classifier?} \fm{I repeated the results selecting the best SKF cross validation results to help distinguish this.}
            \item Incremental learner
            \begin{itemize}
            \item $|V|$, $|E|$, \# HDBSCAN clusters, precision on clusters determined by naive algorithm
            \item $|V|$, $|E|$, \# HDBSCAN clusters, $\sigma$ has same performance

\item classification accuracy: 0.89
\item LOO CV: 0.84
 \item SKF CV: 0.73
            \end{itemize}
          \item I just realized I should probably try this for the \citeA{abbott.etal.2015} network
        \end{enumerate}
    \end{itemize}
    \item cosine patch entry similarity (figure 2)
    \begin{itemize}
        \item Instead of looking at the average IRTs between successive items in the walk, we can also look at the average cosine similarity between words
        \item \citeA{hills.etal.2012} looked at the BEAGLE cosine similarity of the human random walk, observing that the cosine similarity between the first and last words in a patch are on average the lowest, and the first and second the highest
        \item we see roughly this same pattern on our walks as well
    \end{itemize}
    \item IRT type proportions (figure 3)
    \ignore{ \an{Explain what the goal of this experiment is.} }
    \begin{itemize}
        \item Hills et al (2015) seek to better define the nature of what semantically related patches in memory may be, over which foraging-like search processes may occur.
        \item In particular, does a patch include all associations formed between words, or are there strict categorical boundaries separating patches
        \item Patch boundaries can be defined on a series of words in the following different ways: a) categorical - each item in cluster of retrieved words has at least one category in common or b) fluid (associative) - each item in cluster of retrieved words has at least one category in common with previous word, as seen in \Figure{fig:pst}
        \item In Hills et al (2015), 61\% of participants (i.e., 61\% of walks) had categorical-only patch switches. There were 2425 associative/categorical patch switches, and only 134 categorical only. 
        
        \ignore{\item In gold, 1635 associative/categorical patch switches 140 categorical-only switches.}
        
        \item (In our batch learer, only 45\% of the walks have categorical-only patch switches, 3875 associative/categorical patch switches and 128 categorical-only switches). In BEAGLE, 46\% of walks had at least one categorical-only patch switch, with 169 categorical patch switches and 5446 additional associative patch switches. In gold, 66\% of walks had categorical patch switches (more like human data), with 137 categorical patch switches across all walks, and 4072 additional associative patch switches,
        \item for each quartile of the random walk, examine proportion of each type of switch
        \item also examine whether the number of associative switches increases with the quartile, while categorical remain the same
        \item for certain parameters, this is observed on all walks on all networks
    \end{itemize}
    
    \item IRT type duration in our networks (figure 4)
    \begin{itemize}
        \item associative patch switches take longer than categorical and non-switches, suggesting that these represent transitions that they are further away in semantic space
        \item for most parameter settings, even when the IRT pattern is produced, categorical patch switches take longest
        \item in figure 3, for some parameter settings for the gold network, the qualitative relationship seen in the human data (fig 5(a)) is observed. This only occurs when the strong IRT pattern is also observed
        \item not observed for the BEAGLE or learner networks
       \ignore{ \an{How many of each switch type are there?} }
    \end{itemize}
    \item IRT type duration in Nelson association norms (figure 6)
    \begin{itemize}
        \item tried the above on the graph constructed using Nelson association norms in Abbotts, Austerweil and Griffiths (2015) (hereafter referred to as the Nelson Network)
        \item network has no 'animal' node: choose start node randomly
        \item walk length unclear: paper says '2000 simulations' which could either refer to individual walk lengths or to the total number of walks averaged together. I chose a walk length of 65 and 282 walks in total (similar to the parameters used for other walks
        \item network is binarized - so can't repeat cosine similarity analyses on it
        \item (N.B.: some of these issues can be circumvented by building a directed network directly from the Nelson association norms)
        \item IRT results are replicated even for these short walk lengths
        \item IRT type duration also replicated, looks pretty similar to the results obtained on the gold graph (figure 5)
    \end{itemize}
    \item Why the Nelson and gold networks are capable of reproducing the IRT type duration pattern (figure 7)
    \begin{itemize}
        \item I propose that the reason we see, on average, a smaller IRT for categorical only switches is that one of the implicit assumptions of the associative search model is that there are multiple possible associations that have overlapping categorical boundaries
        \item in other words, words belong to more than one category and this is reflected in the way words can be retrieved in humans
        \item at the tau thresholds needed to resolve different animal categories, we eliminate most between-cluster (i.e. between-category) edges in the learner network, evidenced by the number of disconnected components when the node 'animal' is removed
        \item relative to the learner network, the gold network at the same tau thresholds has fewer disconnected components (when 'animal' is removed)
        \item the Nelson network, on the other hand, has only a few disconnected components which are just a few solitary nodes.
    \end{itemize}
    \item Possible ways to construct the gold/learner networks to reflect the IRT duration type pattern
    \begin{itemize}
        \item It makes sense to apply some kind of normalization scheme so that edge weights are scaled proportionately (i.e., when tau is low, only the weakest edges for all nodes are removed). This may help preserve between-category edges to better reflect multiple category membership
        \item Several ways to possibly do this. Notice that in each case a directed graph will be formed.
        \begin{enumerate}
            \item Normalize each edge to the sum of cosine similarities for that word and all other words (or at least all other animal words). Intuitively, since the random walker always transitions to another node in each step of the walk, the sum of the probabilities of choosing an incident edge is 1, regardlesss of the absolute edge weights.
            \begin{itemize}
                \item Formally, assign edge weight from node $b \rightarrow a$ as:
                \begin{align*}
                    P(a|b) &= \frac{Sim(a,b)}{\sum_{i\in N} Sim(b,i) }
                \end{align*}
                \item Where $N$ is the set of all nodes and $Sim$ is a similarity function calculating the cosine similarity of the vector representations of the nodes.
                \item I tried this on the gold network, and I could produce networks that replicated the strong IRT pattern, but none reproduced the IRT duration type pattern.
            \end{itemize}
            \item Rescale the weights to span the interval $(0,1]$ by dividing the weights for a given nodes by maximal weight.
                \begin{align*}
                    P(a|b) &= \frac{Sim(a,b)}{max_{i\in N}( Sim(b,i) )} %\sum_{i\in N} Sim(b,i) }
                \end{align*}
                \begin{itemize}
                    \item  Where $N$ is the set of all nodes and $Sim$ is a similarity function calculating the cosine similarity of the vector representations of the nodes.
                    \item I tried this and could only produce the weak IRT pattern sparsely across the parameter space. The IRT duration type was replicated on a few points, but not always with a graph that reproduced the IRT pattern
                \end{itemize}
               
            \item (New idea, haven't tried this yet:) Filter edge weights at each node by rank, i.e. a tau of 0.5 would remove the weakest $50\%$ of edges at each node
            \item If the IRT type duration behavior isn't observed because the scene-utterance pairs emphasize one possible set of associations between word (rather than multiple ways different words could be related), then exposing the learner to more utterances that capture a broader context of animal word usage should help it represent the multiple categories a word could be associated with.
            \begin{itemize}
                \item I tried training a learner on all 120k utterances in the training set, and then on all animal utterances in the test set. Unfortunately, I still could not capture the IRT duration type pattern observed in humans, Nelson and gold.
            \end{itemize}
        \end{enumerate}
    \end{itemize}
\end{enumerate}




\begin{figure}


\ignore{
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/gold_prop}
  \caption{Gold network}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/adul_prop.png}
  \caption{Batch Learner}
  \label{fig:sfig3}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/BEAGLE_prop.png}
  \caption{BEAGLE network}
  \label{fig:sfig4}
\end{subfigure}
}
\caption{\small{Average IRTs relative to patch entry position normalized to the long-term average.  Bars are SEM.}} %Bars are \todo{SEM}.}
\label{fig:allIRTs}
%\vspace{-0.5cm}
\end{figure}






\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[height=3cm,trim=0 0 10 0, clip,scale=0.35]{550/humanquart.png}
  \caption{Human data }
  \label{fig:hills}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/gold_prop}
  \caption{Gold network}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/adul_prop.png}
  \caption{Batch Learner}
  \label{fig:sfig3}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/BEAGLE_prop.png}
  \caption{BEAGLE network}
  \label{fig:sfig4}
\end{subfigure}
\caption{\small{Average proportion of IRTs based on patch switch type on each quartile of the random walk for (a) human data, reproduced from \citeA{hills.etal.2012}, (b--d) our models on weighted random walks using the parameters described in Comparing Best Results. Bars are SEM.}} %Bars are \todo{SEM}.}
\label{fig:catprop}
%\vspace{-0.5cm}
\end{figure}

\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 10 0, clip,scale=0.35]{550/humandif.png}
  \caption{Human data }
  \label{fig:hills}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/gold_difirt}
  \caption{Gold network}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/adul_difirt.png}
  \caption{Batch Learner}
  \label{fig:sfig3}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/BEAGLE_difirt.png}
  \caption{BEAGLE network}
  \label{fig:sfig4}
\end{subfigure}
\caption{\small{Average IRTs based on patch switch types for (a) human data, reproduced from \citeA{hills.etal.2012}, (b--d) our models on weighted random walks using the parameters described in Comparing Best Results. Bars are SEM.}} %Bars are \todo{SEM}.}
\label{fig:allIRTs}
%\vspace{-0.5cm}
\end{figure}


\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 10 0, clip,scale=0.29]{gold_param}
  \caption{gold parameter space}
  \label{fig:hills}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{figure_16}
  \caption{IRT type duration}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{figure_10}
  \caption{IRT pattern}
  \label{fig:sfig3}
\end{subfigure}%

\ignore{
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.12]{gold_directed_param}
  \caption{gold directed parameter space}
  \label{fig:sfig4}
\end{subfigure}
}

\caption{\small{For certain parameters (a) on the gold network, it is possible to also replicate the qualitative difference between the IRT types (b). %Average IRTs based on patch switch types for (a) human data, reproduced from \citeA{hills.etal.2012}, (b--d) our models on weighted random walks using the parameters described in Comparing Best Results. Bars are SEM.}} %Bars are \todo{SEM}.}
}}
\label{fig:allIRTs}
%\vspace{-0.5cm}
\end{figure}



\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/nelson_irt}
  \caption{IRTs}
  \label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/nelson_difirt}
  \caption{IRT type duration}
  \label{fig:sfig2}
\end{subfigure}
\caption{\small{ For the network used by \citeA{abbott.etal.2015} it is possible to  replicate (a) both the IRT pattern and (b) the qualitative difference between the IRT duration types. %Average IRTs based on patch switch types for (a) human data, reproduced from \citeA{hills.etal.2012}, (b--d) our models on weighted random walks using the parameters described in Comparing Best Results. Bars are SEM.}} %Bars are \todo{SEM}.}
}}
\label{fig:allIRTs}
%\vspace{-0.5cm}
\end{figure}

\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 0, clip,scale=0.05]{550/gold_hillscateg}
  \caption{Gold}
  \label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 0, clip,scale=0.05]{550/adul_hillscateg}
  \caption{Learner network}
  \label{fig:sfig1}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 0, clip,scale=0.05]{550/NELSON_hillscateg}
  \caption{Nelson}
  \label{fig:sfig2}
\end{subfigure}
\caption{\small{ (a) the gold network ($\tau=0.8,\tau_{animal}=0.4$), (b) the non-incremental learner network, and (c) the network used by \citeA{abbott.etal.2015} derived from Nelson association norms. %Average IRTs based on patch switch types for (a) human data, reproduced from \citeA{hills.etal.2012}, (b--d) our models on weighted random walks using the parameters described in Comparing Best Results. Bars are SEM.}} %Bars are \todo{SEM}.}
}}
\label{fig:allGraphs}
%\vspace{-0.5cm}
\end{figure}

\begin{figure}  

\centering
  \includegraphics[trim=0 0 0 0, clip,scale=0.65]{categories}

\ignore{
\begin{subfigure}{.3\textwidth}

  \caption{Gold}
  \label{fig:sfig1}
\end{subfigure}
}

\caption{\small{ The difference between categorical and associative patch switches, reproduced from \citeA{hills.etal.2015}. The topmost circles indicate category memberships defined in \citeA{troyer.etal.1997}. In associative search, a patch switch occurs only when the next word shared no categories in common with the preceding word, as is the case of `wolf' and `cow'. Categorical switches occur if a word doesn't share whichever category is common to the preceding cluster of words. Note that while associative switches are necessarily categorical switches, the reverse needn't be true, in which case it is referred to as a `categorical-only' patch switch. 
}}
\label{fig:pst}
%\vspace{-0.5cm}
\end{figure}

}

%%032
\an{Is categorical/associative just all the categorical switches? And categorical only categorical-associative?}\fm{See figure 1 updated}

\an{Can we relate this to the markov assumption--the number of previous words that effect a switch}\fm{I'm not sure if it matters, strictly speaking only a memory of the words in the current cluster matter (because this is how the cluster category is determined) which is technically unbounded but in actuality is maximally as large as the largest cluster's size}
\an{What I found interesting -- related to the markov assumption -- is that in one type of switch, the participants presumably use more memory; because they need to remember all the words in that patch as opposed to the previous word.} \fm{I think the categorical model requires more memory because you have to keep track of what category is shared by all members in the cluster. In the associative model, you only keep track of the last word's categories compared to the current word. So this may be interesting to add, that the associative model actually potentially has less memory overhead. I think the memoryless-ness of the random walk may go towards explaining why we replicate the findings that the associative model better explains our data.}


%%033

\ignore{
Each model was trained on all networks generated from one semantic source (e.g. gold, BEAGLE, learner) were validated with two cross-validation metrics. We used leave-one out (LOO) cross-validation, where the model is trained on $n$ different partitions of the data of size $n-1$, and the average accuracy with which it classified the $n^{th}$ network is computed. We also used stratified 3-fold (SKF) cross validation (CV), where the data is partitioned into 3 equally-sizes. We report only the models with the highest SKF cross-validation scores.

\subsubsection{Results of Logistic Regression}
\ignore{
\SXS{This next paragraph is very hard to read.  Is there any way to simplify this or put it in a table?} \fm{I included the features that overlap between the models in the table. Because it's kind of wordy to explain some of the models (i.e., there are actually a number of models that perform equally well for the incremental model).} \SXS{Could we make this detail available on github and just report the key features in the table, if we need the space?}
}
For our gold networks, the features that appeared in the logistic regression model that achieved the best cross-validation score were $\lambda$, $\gamma$, weighted F-score, number of clusters determined by HDBSCAN, number of clusters determined by the naive clustering algorithm, precision and F-score (on clusters identified by the naive clustering algorithm). The features in the best model for the learned network were $\gamma$, weighted F-score, and number of singletons. For the incremental network, the features in the best performing logistic regression models were one of  \{$|E|$, $L$, $\lambda$, $\gamma$, sparsity, weighted F-score, the number of clusters identified by the naive clustering algorithm\} plus unweighted F-score of the clusters identified by the naive clustering algorithm. For BEAGLE, the features were L,$\gamma$, and number of clusters determined by HDBSCAN. 

\Table{tab:lr} shows the classification accuracy, cross-validation scores, and list of features that are shared by at least two of the networks.
We note that the normalized clustering coefficient ($\gamma$) is a predictor for all of the networks. Likewise, the weighted or unweighted F-score is a significant predictor for all but the BEAGLE networks. 

The original criterion for small-worldness was defined as $\lambda\approx 1,\gamma\gg1$ \cite{watts.strogatz.1998}, which respectively refer to a low average path length, but high degree of clustering compared to a random network. Across all our networks, the $\gamma$ term varies more than $\lambda$ since $\lambda\approx 1$. The result of the logistic regression suggests that $\gamma$ is predictive of the IRT pattern for all networks. Since $\gamma$ is the dominating term in $\sigma$, this observation is consistent with previous findings regarding small-world structure in semantic networks \cite{steyvers.tenenbaum.2005,nematzadeh.etal.2016}.
However, in addition to the small-worldness criterion, we observe that the weighted F-score is a predictor that occurs for all but the BEAGLE networks. Hence, we conclude that both topological features -- namely, a high clustering coefficient and short average path length -- and semantic features -- good precision and recall in clusters -- are jointly associated with reproducing the IRT pattern.\ignore{ \an{In the table report the SKF and whether a feature form each group was an indicator. So the columns are SKF accuracy, overall structure, etc.}
}
\begin{table}
\begin{center}
\small{
\begin{tabular}{ |l |r |r|}  
%\cline{2-7} 
\ignore{
\multicolumn{1}{c}{}  & \multicolumn{3}{|c|}{Structure} &\multicolumn{3}{|c|}{Semantics} \\ }
\hline
  Network &  SKF & Features in Common \\
\hhline{|=|=|=|}
 Gold  
  & 92 & $\gamma$, F-score,\\&& weighted F-score, $|H|$  \\
 \hline
 Learner & 93 & $\gamma$, weighted F-score \\
 \hline
 Incremental&&\\ learner&  93 & $\gamma$, F-score \\
 \hline
 BEAGLE & 94 & $\gamma$, $|H|$     \\ 
\hline
\end{tabular}
}
\end{center}
\vspace{-0.3cm}
\caption{\small{Performance of best logistic regression models for predicting IRT pattern production. Classification accuracy (CA) over the entire set of networks is also reported.}}
\label{tab:lr}
\vspace{-0.5cm}
\end{table}
}

%%06
 We also show that the learned representations from BEAGLE capture these data equally well when appropriately structured into a thresholded semantic network.
 
 
%\section{The Interplay of Structure and Semantics}
\ignore{
\subsection{Identifying Semantic Clusters}
%\an{Need an intro here too. Say sth about why we care about the structure and semantics of the network. I know you say it later in the section, but it is good to guied the reader why they should care about clustering and logistic regression.}

In previous work \cite{nematzadeh.etal.2016}, we noted that because of the fine-grained distinctions in word meanings our learning model captures, the resulting networks exhibit a star-like structure, with most components connecting to the word `animal'. Clusters can be identified simply by deleting the word `animal' and examining the remaining disconnected components, including singular words. We refer to this as the naive clustering algorithm.

Additionally, we use the HDBSCAN clustering algorithm (hierarchical density-based spatial clustering of applications with noise), with a minimum cluster size of 3 \cite{Campello2013}. Note that unlike our naive clustering algorithm, not all words are assigned to a cluster (notably, components with 3 or fewer nodes).

%\subsection{Logistic Regression on Structural and Semantic Features}
}

==> 07-results_notused.tex <==
\section{Results}
\subsection{Patch Entry Position IRTs and Cosine Similarity}

In the human free recall task (\Figure{fig:hills}), the longest IRT occurs at a patch switch -- where successive words do not share a semantic category -- presumably reflecting the greater distance in semantic memory \cite{hills.etal.2012,hills.etal.2015}. The IRT drops between the first and second items in a patch, then steadily increases until the IRT exceeds the long-term average IRT, again reflecting occurrence of a patch switch. This pattern is replicated on the BEAGLE,  learner, incremental learner and gold (not shown) networks we examined (\Figure{fig:allIRTs}).  


An analogous pattern with respect to patch entry positions is found with the average cosine similarities, although here, because cosine represents similarity rather than distance, the direction is reversed, as seen in \Figure{fig:allcos}. 
Words at a patch switch are the least similar to one another. They are most similar at the beginning of a patch, and then similarity decreases. We note that unlike in BEAGLE, the differences in cosine similarity within a patch much smaller because the threshold applied to our learner is higher. 

%\SXS{The figure doesn't show gold, but does show BEAGLE.} \fm{I'm trying to think whether to include gold or not in the figures - the only thing new about gold in this paper is the cosine similarity pattern and logistic regression. The figures would also take up disproportionately more space (since only two can fit on a line at a time. I couold just make one big figure to save space. Anyways, let me know what you think.}

%\SXS{I think saying ``The opposite pattern'' here is misleading.  It's really the same pattern, it's just opposite because of the measure we use -- ie, larger semantic distance = higher IRT = lower cosine.  Would this work to replace the next sentence:  ``An analogous pattern is found in the average cosine similarities with respect to the patch entry positions, although here, because cosine represents similarity rather than distance, the direction is reversed -- i.e., \Figure{fig:allcos} shows that cosine goes up when IRT goes down, and vice versa.''} \fm{Thanks! I don't want to say that cosine goes up when IRT goes down, because although that does make sense, it's not explicitly clear whether that occurs in the Hills data (note they provide only 5 bars of data rather than 7 in fig 1a). However I can comment on general patterns}
\fm{Figures will need to be resized}
\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[height=3cm,width=4.5cm,trim=0 0 10 47, clip,scale=0.35]{550/hills1.png}
  \caption{Human data }
  \label{fig:hills}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{beagle_irt}
  \caption{BEAGLE network}
  \label{fig:sfig4}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{adul_irt}
  \caption{Learner network}
  \label{fig:sfig3}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{incremental_learner_irt}
  \caption{Incremental network}
  \label{fig:hillsIRT}
\end{subfigure}%
\caption{\small{(a) Human IRTs reproduced from \citeA{hills.etal.2012}.\\(b--d) Modeling IRTs in  weighted random walks using the parameters described in \citeA{nematzadeh.etal.2016}.}} %Bars are \todo{SEM}.}
\label{fig:allIRTs}
%\vspace{-0.5cm}
\vspace{-1em}
\end{figure}

\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[height=3cm,width=4.5cm,trim=0 0 10 0, clip,scale=0.29]{human_cos}
  \caption{Human (on BEAGLE)}
  \label{fig:hillscos}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{BEAGLE_cos}
  \caption{BEAGLE}
  \label{fig:beaglecos}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{adul_cos}
  \caption{Learner}
  \label{fig:sfig3}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{incremental_learner_cos}
  \caption{Incremental learner}
  \label{fig:sfig2}
\end{subfigure}


\caption{\small{Cosine similarities between words in successive patch positions normalized by the average long-term cosine similarity in (a) BEAGLE vectors for items retrieved by humans \cite{hills.etal.2012}, (b-d) our semantic networks.
}}
\label{fig:allcos}
%\vspace{-0.5cm}
\vspace{-1.5em}
\end{figure}





\ignore{
\SXS{Are these the figures for the new results with cosine?}
\SXS{The text needs to be updated to match the actual (new) results.  What this says here, previous and next sentences, doesn't match the current figures, but I think they might be the old ones.} \fm{The figures are the newest ones. I think we should mention why the similarities are so close... thinking about what else to say.}
\SXS{NEW: Ok, I'm going to try again.  The sentence above says our diffs in cos similarity are smaller than BEAGLE, but they're not.  I don't understand what you're trying to say.} 
%\SXS{The differences don't look that different between learner and BEAGLE.  What seems different in the learner is that the cosine continues to increase \textbf{after} a patch switch -- that seems odd to me.  I don't understand how that can happen.} \fm{I think I figured it out! After wracking my brain and painstakingly verifying there were no code bugs (which there weren't!) I realized my intuition that `animal' being compared with another word would bring down the average cosine similarity on the second patch entry position was correct! What I failed to consider is that this will happen at the beginning of EVERY walk in the trial. When I exclude the first cluster retrieved in continuity with `animal', the discrepancy is lessened.} 
%
Note, as mentioned before, that the `human' data in \Figure{fig:hillscos} is calculating cosine similarities over the BEAGLE representations of the words generated by participants in the free recall task; thus the patterns observed in Figures \ref{fig:hillscos} and \ref{fig:beaglecos} may have a strong resemblance since they are using the same vector space.
\SXS{I'm not really sure where this last sentence fits in, or even if it does -- depends on what you say about the match of our models to the human data.}
}


\subsection{Patch Switch Type Proportion and Duration}

\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[height=3cm,width=4.5cm]{550/humanquart.png}
  \caption{Human }
  \label{fig:hills}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{beagle_prop.png}
  \caption{BEAGLE }
  \label{fig:sfig4}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{adul_prop.png}
  \caption{Learner }
  \label{fig:sfig3}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{incremental_learner_prop}
  \caption{Incremental learner}
  \label{fig:sfig2}
\end{subfigure}
\caption{\small{Average proportion of IRTs based on patch switch type on each quartile of the random walk for (a) human data \cite{hills.etal.2012}, (b--d) our semantic networks.}} %Bars are \todo{SEM}.}
\label{fig:catprop}
%\vspace{-0.5cm}
\vspace{-1.2em}
\end{figure}

In \citeA{hills.etal.2015}, 61\% of the walks produced by participants had categorical-only patch switches. As seen in \Figure{fig:catprop}, the distribution of each type of patch switch over the four quartiles of items retrieved is such that associative switches dominate, and increase in frequency as the walk progresses, while categorical-only switches represent a constant, small fraction of all patch switches.

Compared to the average IRT within a patch, associative and categorical-only patch switches take longer (\Figure{fig:irttype}), suggesting that items in different patches are further apart in semantic memory than items within a patch. However, associative patch switches take much longer than both. \citeA{hills.etal.2015} take this as evidence for the associative patch model in semantic memory.


\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[height=3cm,width=4.5cm]{550/humandif.png}
  \caption{Human data }
  \label{fig:hills}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{beagle_irttype}
  \caption{BEAGLE }
  \label{fig:sfig4}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{adul_irttype}
  \caption{Learner }
  \label{fig:sfig3}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{incremental_learner_irttype}
  \caption{Incremental learner}
  \label{fig:sfig2}
\end{subfigure}
\caption{\small{Average IRTs based on patch switch types for (a) human data \cite{hills.etal.2012}, (b--d) our semantic networks.}} %Bars are \todo{SEM}.}
\label{fig:irttype}
%\vspace{-0.5cm}
\vspace{-1.5em}
\end{figure}

We note that although \citeA{hills.etal.2012} found that randomly sampling words without replacement in BEAGLE did not fit the human data, we show  that when the representation is structured into a semantic network and the appropriate threshold for cosine similarity is chosen, it fits the data on all of the measures we investigated as well as our models do.


\subsection{Results of Logistic Regression}
\ignore{
\SXS{This next paragraph is very hard to read.  Is there any way to simplify this or put it in a table?} \fm{I included the features that overlap between the models in the table. Because it's kind of wordy to explain some of the models (i.e., there are actually a number of models that perform equally well for the incremental model).} \SXS{Could we make this detail available on github and just report the key features in the table, if we need the space?}
}
For our gold networks, the features that appeared in the logistic regression model that achieved the best cross-validation score were $\lambda$, $\gamma$, weighted F-score, number of clusters determined by HDBSCAN, number of clusters determined by the naive clustering algorithm, precision and F-score (on clusters identified by the naive clustering algorithm). The features in the best model for the learned network were $\gamma$, weighted F-score, and number of singletons. For the incremental network, the features in the best performing logistic regression models were one of  \{$|E|$, $L$, $\lambda$, $\gamma$, sparsity, weighted F-score, the number of clusters identified by the naive clustering algorithm\} plus unweighted F-score of the clusters identified by the naive clustering algorithm. For BEAGLE, the features were L,$\gamma$, and number of clusters determined by HDBSCAN. 

\Table{tab:lr} shows the classification accuracy, cross-validation scores, and list of features that are shared by at least two of the networks.
We note that the normalized clustering coefficient ($\gamma$) is a predictor for all of the networks. Likewise, the weighted or unweighted F-score is a significant predictor for all but the BEAGLE networks. 

The original criterion for small-worldness was defined as $\lambda\approx 1,\gamma\gg1$ \cite{watts.strogatz.1998}, which respectively refer to a low average path length, but high degree of clustering compared to a random network. Across all our networks, the $\gamma$ term varies more than $\lambda$ since $\lambda\approx 1$. The result of the logistic regression suggests that $\gamma$ is predictive of the IRT pattern for all networks. Since $\gamma$ is the dominating term in $\sigma$, this observation is consistent with previous findings regarding small-world structure in semantic networks \cite{steyvers.tenenbaum.2005,nematzadeh.etal.2016}.
However, in addition to the small-worldness criterion, we observe that the weighted F-score is a predictor that occurs for all but the BEAGLE networks. Hence, we conclude that both topological features -- namely, a high clustering coefficient and short average path length -- and semantic features -- good precision and recall in clusters -- are jointly associated with reproducing the IRT pattern.\ignore{ \an{In the table report the SKF and whether a feature form each group was an indicator. So the columns are SKF accuracy, overall structure, etc.}
}
\begin{table}
\begin{center}
\small{
\begin{tabular}{ |l |r |r|}  
%\cline{2-7} 
\ignore{
\multicolumn{1}{c}{}  & \multicolumn{3}{|c|}{Structure} &\multicolumn{3}{|c|}{Semantics} \\ }
\hline
  Network &  SKF & Features in Common \\
\hhline{|=|=|=|}
 Gold  
  & 92 & $\gamma$, F-score,\\&& weighted F-score, $|H|$  \\
 \hline
 Learner & 93 & $\gamma$, weighted F-score \\
 \hline
 Incremental&&\\ learner&  93 & $\gamma$, F-score \\
 \hline
 BEAGLE & 94 & $\gamma$, $|H|$     \\ 
\hline
\end{tabular}
}
\end{center}
\vspace{-0.3cm}
\caption{\small{Performance of best logistic regression models for predicting IRT pattern production. Classification accuracy (CA) over the entire set of networks is also reported.}}
\label{tab:lr}
\vspace{-0.5cm}
\end{table}

\ignore{

\begin{enumerate}
    \item Performance of incremental networks (figure 1)
    \begin{itemize}
        \item rather than generating the semantic networks on the final learned word vectors, we can update the semantic network online as the model learns
        \item trained on 78k utterances from the training scene/utterance pairs derived from CHILDES
        \item IRT pattern is reproduced
    \end{itemize}
    \item Logistic regression on features
    \begin{itemize}
        \item sample equally from the parameter spaces in which IRT patterns occur and do not occur (so null model classification rate would be $50\%$)
        \item for each of the different models (gold, learner, beagle),  perform logistic regression on all possible combinations of the following features: number of vertices (V), number of edges (E), characteristic path length (L), L normalized to an equivalent Erdos-Renyi graph (lambda), clustering coefficient (CC), CC normalized to an equivalent Erdos-Renyi graph (gamma), sparsity, small-worldness (sigma), adjusted rand index, F-score weighted by cluster sizes, unweighted F-score, number of clusters determined by HDBSCAN, number of clusters determined by the naive clustering algorithm (i.e., deleting the word 'animal' and examining the disconnected components), number of singletons (i.e., number of words that are only connected to 'animal')
        \item examine simplest models that achieve the highest
        \begin{enumerate}
            \item overall classification score - percent of all graphs trained on that are correctly classified as having the IRT pattern or not
            \item true positives score - percent of IRT-producing graphs that are correctly classified (I looked at this separately because initially there were more non-IRT graphs than IRT graphs when the parameter space is unformly sampled)
            \item leave-one-out (LOO) cross-validation score (CV) - make n partitions on the data that leave one graph out, and take the average score of whether that graph is classified correctly or not
            \item stratified k-fold (SKF) cross-validation score - split training data into k equally sized partitions that also capture relative frequencies of each category. Used $k=3$
        \end{enumerate}
        \item Logistic regression results:
        \begin{enumerate}
            \item Gold
            \begin{itemize}
                \item trained on 38 each of IRT and non-IRT graphs
                \item best model: $|E|$, L, $\gamma$, $\sigma$, \# of singletons, precision and F-score (on the naive clustering algorithm)
                \item classification accuracy: 0.96
                \item LOO CV: 0.91
                \item SKF CV: 0.84
                
                \item second best model: $|E|$, L, CC, $\gamma$, $\sigma$, \# of singletons, precision (on the naive clustering algorithm)
                \item classification accuracy: 0.96
                \item LOO CV: 0.91
                \item SKF CV: 0.84
            \end{itemize}
            \item BEAGLE
            \begin{itemize}
                \item trained on 33 each of IRT and non-IRT graphs
                \item best model: $|E|$, weighted F-score (HDBSCAN)
                \item classification accuracy: 0.86
                \item LOO CV: 0.81
                \item SKF CV: 0.69
                \item model with just edges (or edges and sparsity) achieves LOO CV of 0.80, but same classification and SKF score
            \end{itemize}
            \item Learner
            \begin{itemize}
                \item trained on 21 IRT-producing graphs, 21 non-IRT graphs
                \item best model: $|E|$, \# clusters determined by HBDSCAN, \# singletons
                \item classification accuracy: 0.95
                \item LOO CV: 0.95
                \item SKF CV: 0.86
                \item second best model: $|V|$, $|E|$, \# singletons
                \item classification accuracy: 0.95
                \item LOO CV: 0.95
                \item SKF CV: 0.79
            \end{itemize}
              \an{I wonder why the number of edges is enough in predicting the IRT data. I expected CC would be important. Are not we overfitting the classifier?} \fm{I repeated the results selecting the best SKF cross validation results to help distinguish this.}
            \item Incremental learner
            \begin{itemize}
            \item $|V|$, $|E|$, \# HDBSCAN clusters, precision on clusters determined by naive algorithm
            \item $|V|$, $|E|$, \# HDBSCAN clusters, $\sigma$ has same performance

\item classification accuracy: 0.89
\item LOO CV: 0.84
 \item SKF CV: 0.73
            \end{itemize}
          \item I just realized I should probably try this for the \citeA{abbott.etal.2015} network
        \end{enumerate}
    \end{itemize}
    \item cosine patch entry similarity (figure 2)
    \begin{itemize}
        \item Instead of looking at the average IRTs between successive items in the walk, we can also look at the average cosine similarity between words
        \item \citeA{hills.etal.2012} looked at the BEAGLE cosine similarity of the human random walk, observing that the cosine similarity between the first and last words in a patch are on average the lowest, and the first and second the highest
        \item we see roughly this same pattern on our walks as well
    \end{itemize}
    \item IRT type proportions (figure 3)
    \ignore{ \an{Explain what the goal of this experiment is.} }
    \begin{itemize}
        \item Hills et al (2015) seek to better define the nature of what semantically related patches in memory may be, over which foraging-like search processes may occur.
        \item In particular, does a patch include all associations formed between words, or are there strict categorical boundaries separating patches
        \item Patch boundaries can be defined on a series of words in the following different ways: a) categorical - each item in cluster of retrieved words has at least one category in common or b) fluid (associative) - each item in cluster of retrieved words has at least one category in common with previous word, as seen in \Figure{fig:pst}
        \item In Hills et al (2015), 61\% of participants (i.e., 61\% of walks) had categorical-only patch switches. There were 2425 associative patch switches, and only 134 categorical only. 
        
        \ignore{\item In gold, 1635 associative/categorical patch switches 140 categorical-only switches.}
        
        \item (In our learner network, only 45\% of the walks have categorical-only patch switches, 3875 associative/categorical patch switches and 128 categorical-only switches). In BEAGLE, 46\% of walks had at least one categorical-only patch switch, with 169 categorical patch switches and 5446 additional associative patch switches. In gold, 66\% of walks had categorical patch switches (more like human data), with 137 categorical patch switches across all walks, and 4072 additional associative patch switches,
        \item for each quartile of the random walk, examine proportion of each type of switch
        \item also examine whether the number of associative switches increases with the quartile, while categorical remain the same
        \item for certain parameters, this is observed on all walks on all networks
    \end{itemize}
    
    \item IRT type duration in our networks (figure 4)
    \begin{itemize}
        \item associative patch switches take longer than categorical and non-switches, suggesting that these represent transitions that they are further away in semantic space
        \item for most parameter settings, even when the IRT pattern is produced, categorical patch switches take longest
        \item in figure 3, for some parameter settings for the gold network, the qualitative relationship seen in the human data (fig 5(a)) is observed. This only occurs when the strong IRT pattern is also observed
        \item not observed for the BEAGLE or learner networks
       \ignore{ \an{How many of each switch type are there?} }
    \end{itemize}
    \item IRT type duration in Nelson association norms (figure 6)
    \begin{itemize}
        \item tried the above on the graph constructed using Nelson association norms in Abbotts, Austerweil and Griffiths (2015) (hereafter referred to as the Nelson Network)
        \item network has no 'animal' node: choose start node randomly
        \item walk length unclear: paper says '2000 simulations' which could either refer to individual walk lengths or to the total number of walks averaged together. I chose a walk length of 65 and 282 walks in total (similar to the parameters used for other walks
        \item network is binarized - so can't repeat cosine similarity analyses on it
        \item (N.B.: some of these issues can be circumvented by building a directed network directly from the Nelson association norms)
        \item IRT results are replicated even for these short walk lengths
        \item IRT type duration also replicated, looks pretty similar to the results obtained on the gold graph (figure 5)
    \end{itemize}
    \item Why the Nelson and gold networks are capable of reproducing the IRT type duration pattern (figure 7)
    \begin{itemize}
        \item I propose that the reason we see, on average, a smaller IRT for categorical only switches is that one of the implicit assumptions of the associative search model is that there are multiple possible associations that have overlapping categorical boundaries
        \item in other words, words belong to more than one category and this is reflected in the way words can be retrieved in humans
        \item at the tau thresholds needed to resolve different animal categories, we eliminate most between-cluster (i.e. between-category) edges in the learner network, evidenced by the number of disconnected components when the node 'animal' is removed
        \item relative to the learner network, the gold network at the same tau thresholds has fewer disconnected components (when 'animal' is removed)
        \item the Nelson network, on the other hand, has only a few disconnected components which are just a few solitary nodes.
    \end{itemize}
    \item Possible ways to construct the gold/learner networks to reflect the IRT duration type pattern
    \begin{itemize}
        \item It makes sense to apply some kind of normalization scheme so that edge weights are scaled proportionately (i.e., when tau is low, only the weakest edges for all nodes are removed). This may help preserve between-category edges to better reflect multiple category membership
        \item Several ways to possibly do this. Notice that in each case a directed graph will be formed.
        \begin{enumerate}
            \item Normalize each edge to the sum of cosine similarities for that word and all other words (or at least all other animal words). Intuitively, since the random walker always transitions to another node in each step of the walk, the sum of the probabilities of choosing an incident edge is 1, regardlesss of the absolute edge weights.
            \begin{itemize}
                \item Formally, assign edge weight from node $b \rightarrow a$ as:
                \begin{align*}
                    P(a|b) &= \frac{Sim(a,b)}{\sum_{i\in N} Sim(b,i) }
                \end{align*}
                \item Where $N$ is the set of all nodes and $Sim$ is a similarity function calculating the cosine similarity of the vector representations of the nodes.
                \item I tried this on the gold network, and I could produce networks that replicated the strong IRT pattern, but none reproduced the IRT duration type pattern.
            \end{itemize}
            \item Rescale the weights to span the interval $(0,1]$ by dividing the weights for a given nodes by maximal weight.
                \begin{align*}
                    P(a|b) &= \frac{Sim(a,b)}{max_{i\in N}( Sim(b,i) )} %\sum_{i\in N} Sim(b,i) }
                \end{align*}
                \begin{itemize}
                    \item  Where $N$ is the set of all nodes and $Sim$ is a similarity function calculating the cosine similarity of the vector representations of the nodes.
                    \item I tried this and could only produce the weak IRT pattern sparsely across the parameter space. The IRT duration type was replicated on a few points, but not always with a graph that reproduced the IRT pattern
                \end{itemize}
               
            \item (New idea, haven't tried this yet:) Filter edge weights at each node by rank, i.e. a tau of 0.5 would remove the weakest $50\%$ of edges at each node
            \item If the IRT type duration behavior isn't observed because the scene-utterance pairs emphasize one possible set of associations between word (rather than multiple ways different words could be related), then exposing the learner to more utterances that capture a broader context of animal word usage should help it represent the multiple categories a word could be associated with.
            \begin{itemize}
                \item I tried training a learner on all 120k utterances in the training set, and then on all animal utterances in the test set. Unfortunately, I still could not capture the IRT duration type pattern observed in humans, Nelson and gold.
            \end{itemize}
        \end{enumerate}
    \end{itemize}
\end{enumerate}




\begin{figure}


\ignore{
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/gold_prop}
  \caption{Gold network}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/adul_prop.png}
  \caption{Learner network}
  \label{fig:sfig3}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/BEAGLE_prop.png}
  \caption{BEAGLE network}
  \label{fig:sfig4}
\end{subfigure}
}
\caption{\small{Average IRTs relative to patch entry position normalized to the long-term average.  Bars are SEM.}} %Bars are \todo{SEM}.}
\label{fig:allIRTs}
%\vspace{-0.5cm}
\end{figure}






\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[height=3cm,trim=0 0 10 0, clip,scale=0.35]{550/humanquart.png}
  \caption{Human data }
  \label{fig:hills}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/gold_prop}
  \caption{Gold network}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/adul_prop.png}
  \caption{Learner network}
  \label{fig:sfig3}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/BEAGLE_prop.png}
  \caption{BEAGLE network}
  \label{fig:sfig4}
\end{subfigure}
\caption{\small{Average proportion of IRTs based on patch switch type on each quartile of the random walk for (a) human data, reproduced from \citeA{hills.etal.2012}, (b--d) our models on weighted random walks using the parameters described in Comparing Best Results. Bars are SEM.}} %Bars are \todo{SEM}.}
\label{fig:catprop}
%\vspace{-0.5cm}
\end{figure}

\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 10 0, clip,scale=0.35]{550/humandif.png}
  \caption{Human data }
  \label{fig:hills}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/gold_difirt}
  \caption{Gold network}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/adul_difirt.png}
  \caption{Learner network}
  \label{fig:sfig3}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/BEAGLE_difirt.png}
  \caption{BEAGLE network}
  \label{fig:sfig4}
\end{subfigure}
\caption{\small{Average IRTs based on patch switch types for (a) human data, reproduced from \citeA{hills.etal.2012}, (b--d) our models on weighted random walks using the parameters described in Comparing Best Results. Bars are SEM.}} %Bars are \todo{SEM}.}
\label{fig:allIRTs}
%\vspace{-0.5cm}
\end{figure}


\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 10 0, clip,scale=0.29]{gold_param}
  \caption{gold parameter space}
  \label{fig:hills}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{figure_16}
  \caption{IRT type duration}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{figure_10}
  \caption{IRT pattern}
  \label{fig:sfig3}
\end{subfigure}%

\ignore{
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.12]{gold_directed_param}
  \caption{gold directed parameter space}
  \label{fig:sfig4}
\end{subfigure}
}

\caption{\small{For certain parameters (a) on the gold network, it is possible to also replicate the qualitative difference between the IRT types (b). %Average IRTs based on patch switch types for (a) human data, reproduced from \citeA{hills.etal.2012}, (b--d) our models on weighted random walks using the parameters described in Comparing Best Results. Bars are SEM.}} %Bars are \todo{SEM}.}
}}
\label{fig:allIRTs}
%\vspace{-0.5cm}
\end{figure}



\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/nelson_irt}
  \caption{IRTs}
  \label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 28, clip,scale=0.25]{550/nelson_difirt}
  \caption{IRT type duration}
  \label{fig:sfig2}
\end{subfigure}
\caption{\small{ For the network used by \citeA{abbott.etal.2015} it is possible to  replicate (a) both the IRT pattern and (b) the qualitative difference between the IRT duration types. %Average IRTs based on patch switch types for (a) human data, reproduced from \citeA{hills.etal.2012}, (b--d) our models on weighted random walks using the parameters described in Comparing Best Results. Bars are SEM.}} %Bars are \todo{SEM}.}
}}
\label{fig:allIRTs}
%\vspace{-0.5cm}
\end{figure}

\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 0, clip,scale=0.05]{550/gold_hillscateg}
  \caption{Gold}
  \label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 0, clip,scale=0.05]{550/adul_hillscateg}
  \caption{Learner network}
  \label{fig:sfig1}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[trim=0 0 0 0, clip,scale=0.05]{550/NELSON_hillscateg}
  \caption{Nelson}
  \label{fig:sfig2}
\end{subfigure}
\caption{\small{ (a) the gold network ($\tau=0.8,\tau_{animal}=0.4$), (b) the non-incremental learner network, and (c) the network used by \citeA{abbott.etal.2015} derived from Nelson association norms. %Average IRTs based on patch switch types for (a) human data, reproduced from \citeA{hills.etal.2012}, (b--d) our models on weighted random walks using the parameters described in Comparing Best Results. Bars are SEM.}} %Bars are \todo{SEM}.}
}}
\label{fig:allGraphs}
%\vspace{-0.5cm}
\end{figure}

\begin{figure}  

\centering
  \includegraphics[trim=0 0 0 0, clip,scale=0.65]{categories}

\ignore{
\begin{subfigure}{.3\textwidth}

  \caption{Gold}
  \label{fig:sfig1}
\end{subfigure}
}

\caption{\small{ The difference between categorical and associative patch switches, reproduced from \citeA{hills.etal.2015}. The top curly brackets indicate category memberships defined in \citeA{troyer.etal.1997}. In associative search, a patch switch occurs only when the next word shared no categories in common with the preceding word, as is the case of `wolf' and `cow'. Categorical switches occur if a word doesn't share whichever category is common to the preceding cluster of words. Note that while associative switches are necessarily categorical switches, the reverse needn't be true, in which case it is referred to as a `categorical-only' patch switch. 
}}
\label{fig:pst}
%\vspace{-0.5cm}
\end{figure}

}

==> 08-reviews.tex <==
Reviews:

Formality of evaluation. I find it a bit of a pity that the overall evaluation in Section 4.1/4.2 remains completely informal, essentially at the level of "the graphs of human performance and the model look similar". I think there is enough data that it makes sense to perform a correlation analysis or something similar. It's hard to say if the incremental and batch network are meaningfully different or not, and it would also facilitate model comparison by other groups. 

\fm{Done. I added the t-tests that confirm the adherence to marginal value theorem (MVT).}

\an{Also address this:}
(Btw, is there a problem with the graph in Fig 3(a)? It only has 5 bars, while (b) and (c), and Fig 2, have 7 each.)

\fm{This is just how the data are reported in Hills. For consistency, I make those other two plots in figure 3 have 5 bars.}


\fm{Check whether other data analyses can be done. 
-acknowledge the similarity of performance of the two models, but because of the binary nature of the IRT pattern it doesn't necessarily make sense to say if one model is 'better' than the other
- future work may explore in more detail the difference in performance of the two models DONE
In section 4, In particular. refer to our first paper on the adherence to marginal value theorem. (Look into t-test for comparing models for future journal submission) DONE }

- Regarding the batch vs. incremental models: As far as I can see, they do almost exactly equally well. This is not
discussed in the paper; the paper rather makes a point of the incremental nature of human language learning. DONE
While I sympathize with the viewpoint, I think the fact that the batch model does as well needs to be acknowledge and
discussed more than it currently is.

- I find the correlation analysis quite confusing; I think the clarity of this section can be improved a lot.
What exactly is the dependent variable that is predicted?  (5.2 just says "human data"). What are the datapoints?
Why is it appropriate to set up a logistic regression model? That assumes essentially a bimodal distribution (or
strictly binary nature) of the predicted variable. What is accuracy? Is that a predictor, or is it an evaluation of the
correlation model? DONE Finally, what motivated the inclusion of F-Score as a predictor? Isn't it obvious from the
beginning that a better model will make better predictions?

\an{Add to Section 5.2
Go over Quality of semantic connections to address these issues
}
------------------------
Review 4

The study is well grounded in directly relevant (narrower) literature, but could have made citations to/comparisons agains recently popular lexical semantic architectures such as word embeddings, which are also obtained in an incremental fashion.

\fm{
Word2Vec and GloVe
- generalizes to other word representation frameworks
- but we focused on Hills data

- these models are trained on very large corpora, and the update step is an exhaustive update
}

I have two main concerns; first regarding authors reduction of "cognitive plausibility" to "incrementality", and second, the highly supervised (if not arbitrary) way of setting the most important parameters of the model. The proposed algorithm is a network construction model based on contextual semantic similarity, one that with some tweaks and tricks (manual threshold setting/clustering of words/special treatment of hypernym "animal") could be used to output a chain of semantically similar/related words in the order and with the strengths recalled by human subjects. This makes the model too explicit and different from a rather implicit architecture where word similarities/relations/networks emerge from a general learning process with an intuitive objective [function].

% Relate to forgetting
% imposing structure. not a learning solution. future work will investigate whether we can learn these distinctions without these thresholds. Also possibly need a richer representation

I would suggest the authors at least talk about alternative learning mechanisms (such as reinforcement learning) that are established both in developmental psychology and AI.

\fm{
Sure, just say something brief - NOT SURE WHAT TO SAY REALLY, besides that our aim specifically is to model retrieval patterns
}


Also, it would be helpful to make clear why an exhaustive search in retrieval time is not "cognitively plausible"; do we know what happens in brain during learning word relations and recall of them??

\fm{ Find a reference for this - couldn't find this. }

\fm{ Github code link, add instructions and a semantic network. Documentation update. Simple writing script. Picture of a semantic network. DONE - but github will need to be updated }




Appropriateness: 5, 5, 5, 5
Originality: 3, 4, 4, 3
Impact of Ideas or Results: 3, 4, 5, 3
Soundness / Correctness: 4, 4, 5, 4
References / Meaningful Comparison: 4, 4, 5, 4
Clarity: 3, 5, 4, 4
Replicability: 4, 5, 4, 3
Impact of Resources: 1, 1, 1, 1
Overall evaluation: 4, 4, 4, 4
Presentation Format: 1, 2, 2, 2



Presentation Format: 2 (Oral presentation)


